Attn-JGNN: Attention Enhanced Join-Graph Neural Networks

We propose an Attention Enhanced Join-Graph Neural Networks(Attn-JGNN) model for solving #SAT problems, which significantly improves the solving accuracy. Inspired by the Iterative Join Graph Propagation (IJGP) algorithm, Attn-JGNN uses tree decomposition to encode the CNF formula into a join-graph, then performs iterative message passing on the join-graph, and finally approximates the model number by learning partition functions. In order to further improve the accuracy of the solution, we apply the attention mechanism in and between clusters of the join-graphs, which makes Attn-JGNN pay more attention to the key variables and clusters in probabilistic inference, and reduces the redundant calculation. Finally, our experiments show that our Attn-JGNN model achieves better results than other neural network methods.

==> section/references.tex <==
@article{DBLP:journals/fmsd/ClarkeBRZ01,
  author       = {Edmund M. Clarke and
                  Armin Biere and
                  Richard Raimi and
                  Yunshan Zhu},
  title        = {Bounded Model Checking Using Satisfiability Solving},
  journal      = {Formal Methods Syst. Des.},
  volume       = {19},
  number       = {1},
  pages        = {7--34},
  year         = {2001},
  url          = {https://doi.org/10.1023/A:1011276507260},
  doi          = {10.1023/A:1011276507260},
  timestamp    = {Fri, 13 Mar 2020 10:55:19 +0100},
  biburl       = {https://dblp.org/rec/journals/fmsd/ClarkeBRZ01.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @article{DBLP:journals/tcs/IvancicYGGA08,  
 title={Efficient SAT-based bounded model checking for software 
 verification}, 
 volume={404}, 
 url={https://doi.org/10.1016/j.tcs.2008.03.013}, 
 DOI={10.1016/j.tcs.2008.03.013}, 
 number={3}, 
 journal={Theoretical Computer Science}, 
 author={Ivančić, Franjo and Yang, Zijiang and Ganai, Malay K. 
 and Gupta, Aarti and Ashar, Pranav}, 
 year={2008}, 
 month={Sep}, 
 pages={256–274}, 
 language={en-US} 
 }


@inproceedings{DBLP:conf/dac/SilvaS00,
  author       = {Jo{\~{a}}o P. Marques Silva and
                  Karem A. Sakallah},
  editor       = {Giovanni De Micheli},
  title        = {Boolean satisfiability in electronic design automation},
  booktitle    = {Proceedings of the 37th Conference on Design Automation, Los Angeles,
                  CA, USA, June 5-9, 2000},
  pages        = {675--680},
  publisher    = {{ACM}},
  year         = {2000},
  url          = {https://doi.org/10.1145/337292.337611},
  doi          = {10.1145/337292.337611},
  timestamp    = {Tue, 06 Nov 2018 16:58:18 +0100},
  biburl       = {https://dblp.org/rec/conf/dac/SilvaS00.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/fmcad/SheeranSS00,
  author       = {Mary Sheeran and
                  Satnam Singh and
                  Gunnar St{\aa}lmarck},
  editor       = {Warren A. Hunt Jr. and
                  Steven D. Johnson},
  title        = {Checking Safety Properties Using Induction and a SAT-Solver},
  booktitle    = {Formal Methods in Computer-Aided Design, Third International Conference,
                  {FMCAD} 2000, Austin, Texas, USA, November 1-3, 2000, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {1954},
  pages        = {108--125},
  publisher    = {Springer},
  year         = {2000},
  url          = {https://doi.org/10.1007/3-540-40922-X\_8},
  doi          = {10.1007/3-540-40922-X\_8},
  timestamp    = {Tue, 14 May 2019 10:00:54 +0200},
  biburl       = {https://dblp.org/rec/conf/fmcad/SheeranSS00.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @inproceedings{DBLP:conf/aips/DomshlakH06,
  author       = {Carmel Domshlak and
                  J{\"{o}}rg Hoffmann},
  editor       = {Derek Long and
                  Stephen F. Smith and
                  Daniel Borrajo and
                  Lee McCluskey},
  title        = {Fast Probabilistic Planning through Weighted Model Counting},
  booktitle    = {Proceedings of the Sixteenth International Conference on Automated
                  Planning and Scheduling, {ICAPS} 2006, Cumbria, UK, June 6-10, 2006},
  pages        = {243--252},
  publisher    = {{AAAI}},
  year         = {2006},
  url          = {http://www.aaai.org/Library/ICAPS/2006/icaps06-025.php},
  timestamp    = {Fri, 05 Feb 2021 17:14:58 +0100},
  biburl       = {https://dblp.org/rec/conf/aips/DomshlakH06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 

 @article{DBLP:journals/jacm/NieuwenhuisOT06, 
 title={Solving SAT and SAT Modulo Theories},
 volume={53}, 
 url={http://dx.doi.org/10.1145/1217856.1217859}, 
 DOI={10.1145/1217856.1217859},
 number={6}, 
 journal={Journal of the ACM}, 
 publisher={Association for Computing Machinery (ACM)}, 
 author={Nieuwenhuis, Robert and Oliveras, Albert and Tinelli, 
 Cesare}, 
 year={2006}, 
 month={Nov}, 
 pages={937–977}, 
 language={en} 
 }

 @article{DBLP:journals/anor/KrocSS11, 
 title={Leveraging belief propagation, backtrack search, and 
 statistics for model counting}, 
 volume={184}, url={http://dx.doi.org/10.1007/s10479-009-0680- 7}, 
 DOI={10.1007/s10479-009-0680-7}, 
 number={1}, journal={Annals of Operations Research}, 
 publisher={Springer Science and Business Media LLC}, 
 author={Kroc, Lukas and Sabharwal, Ashish and Selman, Bart}, 
 year={2010}, 
 month={Jan}, 
 pages={209–231}, 
 language={en} 
}

 @inproceedings{DBLP:conf/aaai/VaezipoorLWMGSB21,
  author       = {Pashootan Vaezipoor and
                  Gil Lederman and
                  Yuhuai Wu and
                  Chris J. Maddison and
                  Roger B. Grosse and
                  Sanjit A. Seshia and
                  Fahiem Bacchus},
  title        = {Learning Branching Heuristics for Propositional Model Counting},
  booktitle    = {Thirty-Fifth {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2021, Thirty-Third Conference on Innovative Applications of Artificial
                  Intelligence, {IAAI} 2021, The Eleventh Symposium on Educational Advances
                  in Artificial Intelligence, {EAAI} 2021, Virtual Event, February 2-9,
                  2021},
  pages        = {12427--12435},
  publisher    = {{AAAI} Press},
  year         = {2021},
  url          = {https://doi.org/10.1609/aaai.v35i14.17474},
  doi          = {10.1609/AAAI.V35I14.17474},
  timestamp    = {Mon, 04 Sep 2023 16:50:27 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/VaezipoorLWMGSB21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/ijcnn/OzolinsFDGZK22,
  author       = {Emils Ozolins and
                  Karlis Freivalds and
                  Andis Draguns and
                  Eliza Gaile and
                  Ronalds Zakovskis and
                  Sergejs Kozlovics},
  title        = {Goal-Aware Neural {SAT} Solver},
  booktitle    = {International Joint Conference on Neural Networks, {IJCNN} 2022, Padua,
                  Italy, July 18-23, 2022},
  pages        = {1--8},
  publisher    = {{IEEE}},
  year         = {2022},
  url          = {https://doi.org/10.1109/IJCNN55064.2022.9892733},
  doi          = {10.1109/IJCNN55064.2022.9892733},
  timestamp    = {Sat, 31 May 2025 23:10:45 +0200},
  biburl       = {https://dblp.org/rec/conf/ijcnn/OzolinsFDGZK22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/AmizadehMW19,
  author       = {Saeed Amizadeh and
                  Sergiy Matusevych and
                  Markus Weimer},
  title        = {Learning To Solve Circuit-SAT: An Unsupervised Differentiable Approach},
  booktitle    = {7th International Conference on Learning Representations, {ICLR} 2019,
                  New Orleans, LA, USA, May 6-9, 2019},
  publisher    = {OpenReview.net},
  year         = {2019},
  url          = {https://openreview.net/forum?id=BJxgz2R9t7},
  timestamp    = {Thu, 25 Jul 2019 14:25:53 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/AmizadehMW19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1903-01969,
  author       = {Saeed Amizadeh and
                  Sergiy Matusevych and
                  Markus Weimer},
  title        = {{PDP:} {A} General Neural Framework for Learning Constraint Satisfaction
                  Solvers},
  journal      = {CoRR},
  volume       = {abs/1903.01969},
  year         = {2019},
  url          = {http://arxiv.org/abs/1903.01969},
  eprinttype    = {arXiv},
  eprint       = {1903.01969},
  timestamp    = {Sat, 30 Mar 2019 19:27:21 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1903-01969.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{DBLP:conf/nips/LiS22,
  author       = {Zhaoyu Li and
                  Xujie Si},
  editor       = {Sanmi Koyejo and
                  S. Mohamed and
                  A. Agarwal and
                  Danielle Belgrave and
                  K. Cho and
                  A. Oh},
  title        = {NSNet: {A} General Neural Probabilistic Framework for Satisfiability
                  Problems},
  booktitle    = {Advances in Neural Information Processing Systems 35: Annual Conference
                  on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans,
                  LA, USA, November 28 - December 9, 2022},
  year         = {2022},
  url          = {http://papers.nips.cc/paper\_files/paper/2022/hash/a40462acc6959034c6aa6dfb8e696415-Abstract-Conference.html},
  timestamp    = {Mon, 08 Jan 2024 16:31:36 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/LiS22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/KuckCTLSSE20,
  author       = {Jonathan Kuck and
                  Shuvam Chakraborty and
                  Hao Tang and
                  Rachel Luo and
                  Jiaming Song and
                  Ashish Sabharwal and
                  Stefano Ermon},
  editor       = {Hugo Larochelle and
                  Marc'Aurelio Ranzato and
                  Raia Hadsell and
                  Maria{-}Florina Balcan and
                  Hsuan{-}Tien Lin},
  title        = {Belief Propagation Neural Networks},
  booktitle    = {Advances in Neural Information Processing Systems 33: Annual Conference
                  on Neural Information Processing Systems 2020, NeurIPS 2020, December
                  6-12, 2020, virtual},
  year         = {2020},
  url          = {https://proceedings.neurips.cc/paper/2020/hash/07217414eb3fbe24d4e5b6cafb91ca18-Abstract.html},
  timestamp    = {Tue, 31 Jan 2023 08:49:48 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/KuckCTLSSE20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tkde/WuLL24,
  author       = {Fang Wu and
                  Siyuan Li and
                  Stan Z. Li},
  title        = {Discovering the Representation Bottleneck of Graph Neural Networks},
  journal      = {{IEEE} Trans. Knowl. Data Eng.},
  volume       = {36},
  number       = {12},
  pages        = {7998--8008},
  year         = {2024},
  url          = {https://doi.org/10.1109/TKDE.2024.3446584},
  doi          = {10.1109/TKDE.2024.3446584},
  timestamp    = {Tue, 28 Jan 2025 08:07:26 +0100},
  biburl       = {https://dblp.org/rec/journals/tkde/WuLL24.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/uai/DechterKM02,
  author       = {Rina Dechter and
                  Kalev Kask and
                  Robert Mateescu},
  editor       = {Adnan Darwiche and
                  Nir Friedman},
  title        = {Iterative Join-Graph Propagation},
  booktitle    = {{UAI} '02, Proceedings of the 18th Conference in Uncertainty in Artificial
                  Intelligence, University of Alberta, Edmonton, Alberta, Canada, August
                  1-4, 2002},
  pages        = {128--136},
  publisher    = {Morgan Kaufmann},
  year         = {2002},
  url          = {https://dslpitt.org/uai/displayArticleDetails.jsp?mmnu=1\&smnu=2\&article\_id=853\&proceeding\_id=18},
  timestamp    = {Wed, 03 Feb 2021 11:09:13 +0100},
  biburl       = {https://dblp.org/rec/conf/uai/DechterKM02.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/corr/abs-2403-12106,
  author       = {Vincent Bouttier and
                  Renaud Jardri and
                  Sophie Den{\`{e}}ve},
  title        = {Circular Belief Propagation for Approximate Probabilistic Inference},
  journal      = {CoRR},
  volume       = {abs/2403.12106},
  year         = {2024},
  url          = {https://doi.org/10.48550/arXiv.2403.12106},
  doi          = {10.48550/ARXIV.2403.12106},
  eprinttype    = {arXiv},
  eprint       = {2403.12106},
  timestamp    = {Mon, 08 Apr 2024 18:24:51 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2403-12106.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cp/DudekPV20,
  author       = {Jeffrey M. Dudek and
                  Vu H. N. Phan and
                  Moshe Y. Vardi},
  editor       = {Helmut Simonis},
  title        = {{DPMC:} Weighted Model Counting by Dynamic Programming on Project-Join
                  Trees},
  booktitle    = {Principles and Practice of Constraint Programming - 26th International
                  Conference, {CP} 2020, Louvain-la-Neuve, Belgium, September 7-11,
                  2020, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {12333},
  pages        = {211--230},
  publisher    = {Springer},
  year         = {2020},
  url          = {https://doi.org/10.1007/978-3-030-58475-7\_13},
  doi          = {10.1007/978-3-030-58475-7\_13},
  timestamp    = {Tue, 08 Sep 2020 19:28:09 +0200},
  biburl       = {https://dblp.org/rec/conf/cp/DudekPV20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tkde/BrauwersF23,
  author       = {Gianni Brauwers and
                  Flavius Frasincar},
  title        = {A General Survey on Attention Mechanisms in Deep Learning},
  journal      = {{IEEE} Trans. Knowl. Data Eng.},
  volume       = {35},
  number       = {4},
  pages        = {3279--3298},
  year         = {2023},
  url          = {https://doi.org/10.1109/TKDE.2021.3126456},
  doi          = {10.1109/TKDE.2021.3126456},
  timestamp    = {Tue, 28 Mar 2023 19:49:56 +0200},
  biburl       = {https://dblp.org/rec/journals/tkde/BrauwersF23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @inproceedings{DBLP:conf/naacl/YangYDHSH16,
  author       = {Zichao Yang and
                  Diyi Yang and
                  Chris Dyer and
                  Xiaodong He and
                  Alexander J. Smola and
                  Eduard H. Hovy},
  editor       = {Kevin Knight and
                  Ani Nenkova and
                  Owen Rambow},
  title        = {Hierarchical Attention Networks for Document Classification},
  booktitle    = {{NAACL} {HLT} 2016, The 2016 Conference of the North American Chapter
                  of the Association for Computational Linguistics: Human Language Technologies,
                  San Diego California, USA, June 12-17, 2016},
  pages        = {1480--1489},
  publisher    = {The Association for Computational Linguistics},
  year         = {2016},
  url          = {https://doi.org/10.18653/v1/n16-1174},
  doi          = {10.18653/V1/N16-1174},
  timestamp    = {Sat, 31 May 2025 23:11:36 +0200},
  biburl       = {https://dblp.org/rec/conf/naacl/YangYDHSH16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}



 @article{Bethe_1997_07,
 title={Statistical Theory of Superlattices},
 volume={150}, 
 url={https://doi.org/10.1098/rspa.1935.0122}, 
 DOI={10.1098/rspa.1935.0122}, 
 number={871}, 
 journal={ Series A - Mathematical and Physical Sciences}, 
 author={Bethe, HansA.}, 
 pages={552–575}, 
 language={en-US},
 year={n.d.}
 }

@article{DBLP:journals/siamdm/ChandrasekaranCGSS11,
  author       = {Venkat Chandrasekaran and
                  Misha Chertkov and
                  David Gamarnik and
                  Devavrat Shah and
                  Jinwoo Shin},
  title        = {Counting Independent Sets Using the Bethe Approximation},
  journal      = {{SIAM} J. Discret. Math.},
  volume       = {25},
  number       = {2},
  pages        = {1012--1034},
  year         = {2011},
  url          = {https://doi.org/10.1137/090767145},
  doi          = {10.1137/090767145},
  timestamp    = {Sat, 25 Apr 2020 13:56:07 +0200},
  biburl       = {https://dblp.org/rec/journals/siamdm/ChandrasekaranCGSS11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/SoosM19,
  author       = {Mate Soos and
                  Kuldeep S. Meel},
  title        = {{BIRD:} Engineering an Efficient {CNF-XOR} {SAT} Solver and Its Applications
                  to Approximate Model Counting},
  booktitle    = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2019, The Thirty-First Innovative Applications of Artificial Intelligence
                  Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
                  Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
                  USA, January 27 - February 1, 2019},
  pages        = {1592--1599},
  publisher    = {{AAAI} Press},
  year         = {2019},
  url          = {https://doi.org/10.1609/aaai.v33i01.33011592},
  doi          = {10.1609/AAAI.V33I01.33011592},
  timestamp    = {Mon, 04 Sep 2023 12:29:24 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/SoosM19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ai/MuiseMBH12,
  author       = {Christian J. Muise and
                  Sheila A. McIlraith and
                  J. Christopher Beck and
                  Eric I. Hsu},
  editor       = {Leila Kosseim and
                  Diana Inkpen},
  title        = {Dsharp: Fast d-DNNF Compilation with sharpSAT},
  booktitle    = {Advances in Artificial Intelligence - 25th Canadian Conference on
                  Artificial Intelligence, Canadian {AI} 2012, Toronto, ON, Canada,
                  May 28-30, 2012. Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {7310},
  pages        = {356--361},
  publisher    = {Springer},
  year         = {2012},
  url          = {https://doi.org/10.1007/978-3-642-30353-1\_36},
  doi          = {10.1007/978-3-642-30353-1\_36},
  timestamp    = {Thu, 28 Sep 2023 12:27:13 +0200},
  biburl       = {https://dblp.org/rec/conf/ai/MuiseMBH12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sat/AchlioptasHT18a,
  author       = {Dimitris Achlioptas and
                  Zayd Hammoudeh and
                  Panos Theodoropoulos},
  editor       = {Olaf Beyersdorff and
                  Christoph M. Wintersteiger},
  title        = {Fast and Flexible Probabilistic Model Counting},
  booktitle    = {Theory and Applications of Satisfiability Testing - {SAT} 2018 - 21st
                  International Conference, {SAT} 2018, Held as Part of the Federated
                  Logic Conference, FloC 2018, Oxford, UK, July 9-12, 2018, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {10929},
  pages        = {148--164},
  publisher    = {Springer},
  year         = {2018},
  url          = {https://doi.org/10.1007/978-3-319-94144-8\_10},
  doi          = {10.1007/978-3-319-94144-8\_10},
  timestamp    = {Mon, 16 Sep 2019 15:30:17 +0200},
  biburl       = {https://dblp.org/rec/conf/sat/AchlioptasHT18a.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sat/Thurley06,
  author       = {Marc Thurley},
  editor       = {Armin Biere and
                  Carla P. Gomes},
  title        = {sharpSAT - Counting Models with Advanced Component Caching and Implicit
                  {BCP}},
  booktitle    = {Theory and Applications of Satisfiability Testing - {SAT} 2006, 9th
                  International Conference, Seattle, WA, USA, August 12-15, 2006, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {4121},
  pages        = {424--429},
  publisher    = {Springer},
  year         = {2006},
  url          = {https://doi.org/10.1007/11814948\_38},
  doi          = {10.1007/11814948\_38},
  timestamp    = {Tue, 14 May 2019 10:00:41 +0200},
  biburl       = {https://dblp.org/rec/conf/sat/Thurley06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/DudekPV20,
  author       = {Jeffrey M. Dudek and
                  Vu Phan and
                  Moshe Y. Vardi},
  title        = {{ADDMC:} Weighted Model Counting with Algebraic Decision Diagrams},
  booktitle    = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2020, The Thirty-Second Innovative Applications of Artificial Intelligence
                  Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
                  Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
                  February 7-12, 2020},
  pages        = {1468--1476},
  publisher    = {{AAAI} Press},
  year         = {2020},
  url          = {https://doi.org/10.1609/aaai.v34i02.5505},
  doi          = {10.1609/AAAI.V34I02.5505},
  timestamp    = {Mon, 04 Sep 2023 16:50:24 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/DudekPV20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @article{DBLP:journals/corr/abs-2202-10025,
  author       = {Yong Lai and
                  Kuldeep S. Meel and
                  Roland H. C. Yap},
  title        = {{CCDD:} {A} Tractable Representation for Model Counting and Uniform
                  Sampling},
  journal      = {CoRR},
  volume       = {abs/2202.10025},
  year         = {2022},
  url          = {https://arxiv.org/abs/2202.10025},
  eprinttype    = {arXiv},
  eprint       = {2202.10025},
  timestamp    = {Wed, 23 Jul 2025 19:36:41 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2202-10025.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/LaiMY21,
  author       = {Yong Lai and
                  Kuldeep S. Meel and
                  Roland H. C. Yap},
  title        = {The Power of Literal Equivalence in Model Counting},
  booktitle    = {Thirty-Fifth {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2021, Thirty-Third Conference on Innovative Applications of Artificial
                  Intelligence, {IAAI} 2021, The Eleventh Symposium on Educational Advances
                  in Artificial Intelligence, {EAAI} 2021, Virtual Event, February 2-9,
                  2021},
  pages        = {3851--3859},
  publisher    = {{AAAI} Press},
  year         = {2021},
  url          = {https://doi.org/10.1609/aaai.v35i5.16503},
  doi          = {10.1609/AAAI.V35I5.16503},
  timestamp    = {Wed, 23 Jul 2025 19:36:41 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/LaiMY21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/SelsamLBLMD19,
  author       = {Daniel Selsam and
                  Matthew Lamm and
                  Benedikt B{\"{u}}nz and
                  Percy Liang and
                  Leonardo de Moura and
                  David L. Dill},
  title        = {Learning a {SAT} Solver from Single-Bit Supervision},
  booktitle    = {7th International Conference on Learning Representations, {ICLR} 2019,
                  New Orleans, LA, USA, May 6-9, 2019},
  publisher    = {OpenReview.net},
  year         = {2019},
  url          = {https://openreview.net/forum?id=HJMC\_iA5tm},
  timestamp    = {Thu, 29 Sep 2022 08:36:56 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/SelsamLBLMD19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @article{DBLP:journals/corr/abs-2012-14873,
  author       = {Sebastian Johann Wetzel and
                  Kevin Ryczko and
                  Roger G. Melko and
                  Isaac Tamblyn},
  title        = {Twin Neural Network Regression},
  journal      = {CoRR},
  volume       = {abs/2012.14873},
  year         = {2020},
  url          = {https://arxiv.org/abs/2012.14873},
  eprinttype    = {arXiv},
  eprint       = {2012.14873},
  timestamp    = {Fri, 08 Jan 2021 17:23:09 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2012-14873.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/esann/Saveri22,
  author       = {Gaia Saveri},
  title        = {Graph Neural Networks for Propositional Model Counting},
  booktitle    = {30th European Symposium on Artificial Neural Networks, Computational
                  Intelligence and Machine Learning, {ESANN} 2022, Bruges, Belgium,
                  October 5-7, 2022},
  year         = {2022},
  url          = {https://doi.org/10.14428/esann/2022.ES2022-88},
  doi          = {10.14428/ESANN/2022.ES2022-88},
  timestamp    = {Mon, 22 May 2023 16:42:56 +0200},
  biburl       = {https://dblp.org/rec/conf/esann/Saveri22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@mastersthesis { 1023549391.nh,
author = { Yifan Zhang },
title = {Research on Model Counting Methods Based on Machine Learning},
school = {Jilin University},
year = {2023}
}

@inproceedings{DBLP:conf/aaai/LaiMY23,
  author       = {Yong Lai and
                  Kuldeep S. Meel and
                  Roland H. C. Yap},
  editor       = {Brian Williams and
                  Yiling Chen and
                  Jennifer Neville},
  title        = {Fast Converging Anytime Model Counting},
  booktitle    = {Thirty-Seventh {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2023, Thirty-Fifth Conference on Innovative Applications of Artificial
                  Intelligence, {IAAI} 2023, Thirteenth Symposium on Educational Advances
                  in Artificial Intelligence, {EAAI} 2023, Washington, DC, USA, February
                  7-14, 2023},
  pages        = {4025--4034},
  publisher    = {{AAAI} Press},
  year         = {2023},
  url          = {https://doi.org/10.1609/aaai.v37i4.25517},
  doi          = {10.1609/AAAI.V37I4.25517},
  timestamp    = {Wed, 23 Jul 2025 19:36:41 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/LaiMY23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cav/LaiMY25,
  author       = {Yong Lai and
                  Kuldeep S. Meel and
                  Roland H. C. Yap},
  editor       = {Ruzica Piskac and
                  Zvonimir Rakamaric},
  title        = {Panini: An Efficient and Flexible Knowledge Compiler},
  booktitle    = {Computer Aided Verification - 37th International Conference, {CAV}
                  2025, Zagreb, Croatia, July 23-25, 2025, Proceedings, Part {III}},
  series       = {Lecture Notes in Computer Science},
  volume       = {15933},
  pages        = {92--105},
  publisher    = {Springer},
  year         = {2025},
  url          = {https://doi.org/10.1007/978-3-031-98682-6\_6},
  doi          = {10.1007/978-3-031-98682-6\_6},
  timestamp    = {Sat, 09 Aug 2025 12:14:22 +0200},
  biburl       = {https://dblp.org/rec/conf/cav/LaiMY25.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/jetai/LvZXZL24,
  author       = {Shuai L{\"{u}} and
                  Tongbo Zhang and
                  Yue Xu and
                  Wenbo Zhou and
                  Yong Lai},
  title        = {Combining bounded solving and controllable randomization for approximate
                  model counting},
  journal      = {J. Exp. Theor. Artif. Intell.},
  volume       = {36},
  number       = {7},
  pages        = {1075--1088},
  year         = {2024},
  url          = {https://doi.org/10.1080/0952813x.2022.2122588},
  doi          = {10.1080/0952813X.2022.2122588},
  timestamp    = {Wed, 23 Jul 2025 19:36:41 +0200},
  biburl       = {https://dblp.org/rec/journals/jetai/LvZXZL24.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ecai/Darwiche04,
  author       = {Adnan Darwiche},
  editor       = {Ram{\'{o}}n L{\'{o}}pez de M{\'{a}}ntaras and
                  Lorenza Saitta},
  title        = {New Advances in Compiling {CNF} into Decomposable Negation Normal
                  Form},
  booktitle    = {Proceedings of the 16th Eureopean Conference on Artificial Intelligence,
                  ECAI'2004, including Prestigious Applicants of Intelligent Systems,
                  {PAIS} 2004, Valencia, Spain, August 22-27, 2004},
  pages        = {328--332},
  publisher    = {{IOS} Press},
  year         = {2004},
  timestamp    = {Fri, 11 May 2018 12:42:30 +0200},
  biburl       = {https://dblp.org/rec/conf/ecai/Darwiche04.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/ijcai/LagniezM17,
  author       = {Jean{-}Marie Lagniez and
                  Pierre Marquis},
  editor       = {Carles Sierra},
  title        = {An Improved Decision-DNNF Compiler},
  booktitle    = {Proceedings of the Twenty-Sixth International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2017, Melbourne, Australia, August
                  19-25, 2017},
  pages        = {667--673},
  publisher    = {ijcai.org},
  year         = {2017},
  url          = {https://doi.org/10.24963/ijcai.2017/93},
  doi          = {10.24963/IJCAI.2017/93},
  timestamp    = {Tue, 20 Aug 2019 16:17:27 +0200},
  biburl       = {https://dblp.org/rec/conf/ijcai/LagniezM17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ijcai/SharmaRSM19,
  author       = {Shubham Sharma and
                  Subhajit Roy and
                  Mate Soos and
                  Kuldeep S. Meel},
  editor       = {Sarit Kraus},
  title        = {{GANAK:} {A} Scalable Probabilistic Exact Model Counter},
  booktitle    = {Proceedings of the Twenty-Eighth International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
                  2019},
  pages        = {1169--1176},
  publisher    = {ijcai.org},
  year         = {2019},
  url          = {https://doi.org/10.24963/ijcai.2019/163},
  doi          = {10.24963/IJCAI.2019/163},
  timestamp    = {Tue, 15 Oct 2024 16:43:28 +0200},
  biburl       = {https://dblp.org/rec/conf/ijcai/SharmaRSM19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/uai/ErmonGS12,
  author       = {Stefano Ermon and
                  Carla P. Gomes and
                  Bart Selman},
  editor       = {Nando de Freitas and
                  Kevin P. Murphy},
  title        = {Uniform Solution Sampling Using a Constraint Solver As an Oracle},
  booktitle    = {Proceedings of the Twenty-Eighth Conference on Uncertainty in Artificial
                  Intelligence, Catalina Island, CA, USA, August 14-18, 2012},
  pages        = {255--264},
  publisher    = {{AUAI} Press},
  year         = {2012},
  url          = {https://dslpitt.org/uai/displayArticleDetails.jsp?mmnu=1\&smnu=2\&article\_id=2288\&proceeding\_id=28},
  timestamp    = {Mon, 23 Nov 2020 08:36:49 +0100},
  biburl       = {https://dblp.org/rec/conf/uai/ErmonGS12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ai/GogateD11,
  author       = {Vibhav Gogate and
                  Rina Dechter},
  title        = {SampleSearch: Importance sampling in presence of determinism},
  journal      = {Artif. Intell.},
  volume       = {175},
  number       = {2},
  pages        = {694--729},
  year         = {2011},
  url          = {https://doi.org/10.1016/j.artint.2010.10.009},
  doi          = {10.1016/J.ARTINT.2010.10.009},
  timestamp    = {Tue, 07 May 2024 20:26:20 +0200},
  biburl       = {https://dblp.org/rec/journals/ai/GogateD11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cp/ChakrabortyMV13,
  author       = {Supratik Chakraborty and
                  Kuldeep S. Meel and
                  Moshe Y. Vardi},
  editor       = {Christian Schulte},
  title        = {A Scalable Approximate Model Counter},
  booktitle    = {Principles and Practice of Constraint Programming - 19th International
                  Conference, {CP} 2013, Uppsala, Sweden, September 16-20, 2013. Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {8124},
  pages        = {200--216},
  publisher    = {Springer},
  year         = {2013},
  url          = {https://doi.org/10.1007/978-3-642-40627-0\_18},
  doi          = {10.1007/978-3-642-40627-0\_18},
  timestamp    = {Tue, 14 May 2019 10:00:45 +0200},
  biburl       = {https://dblp.org/rec/conf/cp/ChakrabortyMV13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ijcai/ChakrabortyMV16,
  author       = {Supratik Chakraborty and
                  Kuldeep S. Meel and
                  Moshe Y. Vardi},
  editor       = {Subbarao Kambhampati},
  title        = {Algorithmic Improvements in Approximate Counting for Probabilistic
                  Inference: From Linear to Logarithmic {SAT} Calls},
  booktitle    = {Proceedings of the Twenty-Fifth International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2016, New York, NY, USA, 9-15 July
                  2016},
  pages        = {3569--3576},
  publisher    = {{IJCAI/AAAI} Press},
  year         = {2016},
  url          = {http://www.ijcai.org/Abstract/16/503},
  timestamp    = {Tue, 20 Aug 2019 16:19:10 +0200},
  biburl       = {https://dblp.org/rec/conf/ijcai/ChakrabortyMV16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cav/SoosGM20,
  author       = {Mate Soos and
                  Stephan Gocht and
                  Kuldeep S. Meel},
  editor       = {Shuvendu K. Lahiri and
                  Chao Wang},
  title        = {Tinted, Detached, and Lazy {CNF-XOR} Solving and Its Applications
                  to Counting and Sampling},
  booktitle    = {Computer Aided Verification - 32nd International Conference, {CAV}
                  2020, Los Angeles, CA, USA, July 21-24, 2020, Proceedings, Part {I}},
  series       = {Lecture Notes in Computer Science},
  volume       = {12224},
  pages        = {463--484},
  publisher    = {Springer},
  year         = {2020},
  url          = {https://doi.org/10.1007/978-3-030-53288-8\_22},
  doi          = {10.1007/978-3-030-53288-8\_22},
  timestamp    = {Wed, 12 Aug 2020 15:15:44 +0200},
  biburl       = {https://dblp.org/rec/conf/cav/SoosGM20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cav/YangM23,
  author       = {Jiong Yang and
                  Kuldeep S. Meel},
  editor       = {Constantin Enea and
                  Akash Lal},
  title        = {Rounding Meets Approximate Model Counting},
  booktitle    = {Computer Aided Verification - 35th International Conference, {CAV}
                  2023, Paris, France, July 17-22, 2023, Proceedings, Part {II}},
  series       = {Lecture Notes in Computer Science},
  volume       = {13965},
  pages        = {132--162},
  publisher    = {Springer},
  year         = {2023},
  url          = {https://doi.org/10.1007/978-3-031-37703-7\_7},
  doi          = {10.1007/978-3-031-37703-7\_7},
  timestamp    = {Tue, 12 Sep 2023 07:57:21 +0200},
  biburl       = {https://dblp.org/rec/conf/cav/YangM23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ai/Roth96,
  author       = {Dan Roth},
  title        = {On the Hardness of Approximate Reasoning},
  journal      = {Artif. Intell.},
  volume       = {82},
  number       = {1-2},
  pages        = {273--302},
  year         = {1996},
  url          = {https://doi.org/10.1016/0004-3702(94)00092-1},
  doi          = {10.1016/0004-3702(94)00092-1},
  timestamp    = {Fri, 05 Sep 2025 18:14:04 +0200},
  biburl       = {https://dblp.org/rec/journals/ai/Roth96.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ai/ChaviraD08,
  author       = {Mark Chavira and
                  Adnan Darwiche},
  title        = {On probabilistic inference by weighted model counting},
  journal      = {Artif. Intell.},
  volume       = {172},
  number       = {6-7},
  pages        = {772--799},
  year         = {2008},
  url          = {https://doi.org/10.1016/j.artint.2007.11.002},
  doi          = {10.1016/J.ARTINT.2007.11.002},
  timestamp    = {Sat, 27 May 2017 14:24:42 +0200},
  biburl       = {https://dblp.org/rec/journals/ai/ChaviraD08.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/ftdb/BroeckS17,
  author       = {Guy Van den Broeck and
                  Dan Suciu},
  title        = {Query Processing on Probabilistic Data: {A} Survey},
  journal      = {Found. Trends Databases},
  volume       = {7},
  number       = {3-4},
  pages        = {197--341},
  year         = {2017},
  url          = {https://doi.org/10.1561/1900000052},
  doi          = {10.1561/1900000052},
  timestamp    = {Mon, 05 Feb 2024 20:26:47 +0100},
  biburl       = {https://dblp.org/rec/journals/ftdb/BroeckS17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tplp/FierensBRSGTJR15,
  author       = {Daan Fierens and
                  Guy Van den Broeck and
                  Joris Renkens and
                  Dimitar Sht. Shterionov and
                  Bernd Gutmann and
                  Ingo Thon and
                  Gerda Janssens and
                  Luc De Raedt},
  title        = {Inference and learning in probabilistic logic programs using weighted
                  Boolean formulas},
  journal      = {Theory Pract. Log. Program.},
  volume       = {15},
  number       = {3},
  pages        = {358--401},
  year         = {2015},
  url          = {https://doi.org/10.1017/S1471068414000076},
  doi          = {10.1017/S1471068414000076},
  timestamp    = {Mon, 26 Oct 2020 08:22:48 +0100},
  biburl       = {https://dblp.org/rec/journals/tplp/FierensBRSGTJR15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ccs/BalutaSSMS19,
  author       = {Teodora Baluta and
                  Shiqi Shen and
                  Shweta Shinde and
                  Kuldeep S. Meel and
                  Prateek Saxena},
  editor       = {Lorenzo Cavallaro and
                  Johannes Kinder and
                  XiaoFeng Wang and
                  Jonathan Katz},
  title        = {Quantitative Verification of Neural Networks and Its Security Applications},
  booktitle    = {Proceedings of the 2019 {ACM} {SIGSAC} Conference on Computer and
                  Communications Security, {CCS} 2019, London, UK, November 11-15, 2019},
  pages        = {1249--1264},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3319535.3354245},
  doi          = {10.1145/3319535.3354245},
  timestamp    = {Sun, 02 Oct 2022 15:56:15 +0200},
  biburl       = {https://dblp.org/rec/conf/ccs/BalutaSSMS19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/siamcomp/Valiant79,
  author       = {Leslie G. Valiant},
  title        = {The Complexity of Enumeration and Reliability Problems},
  journal      = {{SIAM} J. Comput.},
  volume       = {8},
  number       = {3},
  pages        = {410--421},
  year         = {1979},
  url          = {https://doi.org/10.1137/0208032},
  doi          = {10.1137/0208032},
  timestamp    = {Wed, 14 Nov 2018 10:45:08 +0100},
  biburl       = {https://dblp.org/rec/journals/siamcomp/Valiant79.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/GomesSS06,
  author       = {Carla P. Gomes and
                  Ashish Sabharwal and
                  Bart Selman},
  title        = {Model Counting: {A} New Strategy for Obtaining Good Bounds},
  booktitle    = {Proceedings, The Twenty-First National Conference on Artificial Intelligence
                  and the Eighteenth Innovative Applications of Artificial Intelligence
                  Conference, July 16-20, 2006, Boston, Massachusetts, {USA}},
  pages        = {54--61},
  publisher    = {{AAAI} Press},
  year         = {2006},
  url          = {http://www.aaai.org/Library/AAAI/2006/aaai06-009.php},
  timestamp    = {Tue, 05 Sep 2023 09:10:47 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/GomesSS06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ijcai/GomesHSS07,
  author       = {Carla P. Gomes and
                  J{\"{o}}rg Hoffmann and
                  Ashish Sabharwal and
                  Bart Selman},
  editor       = {Manuela M. Veloso},
  title        = {From Sampling to Model Counting},
  booktitle    = {{IJCAI} 2007, Proceedings of the 20th International Joint Conference
                  on Artificial Intelligence, Hyderabad, India, January 6-12, 2007},
  pages        = {2293--2299},
  year         = {2007},
  url          = {http://ijcai.org/Proceedings/07/Papers/369.pdf},
  timestamp    = {Tue, 20 Aug 2019 16:18:58 +0200},
  biburl       = {https://dblp.org/rec/conf/ijcai/GomesHSS07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
